Spreadsheet Probabilistic Programming

Spreadsheet workbook contents are simple programs. Because of this, probabilistic programming techniques can be used to perform Bayesian inversion of spreadsheet computations. What is more, existing execution engines in spreadsheet applications such as Microsoft Excel can be made to do this using only built-in functionality. We demonstrate this by developing a native Excel implementation of both a particle Markov Chain Monte Carlo variant and black-box variational inference for spreadsheet probabilistic programming. The resulting engine performs probabilistically coherent inference over spreadsheet computations, notably including spreadsheets that include user-defined black-box functions. Spreadsheet engines that choose to integrate the functionality we describe in this paper will give their users the ability to both easily develop probabilistic models and maintain them over time by including actuals via a simple user-interface mechanism. For spreadsheet end-users this would mean having access to efficient and probabilistically coherent probabilistic modeling and inference for use in all kinds of decision making under uncertainty.

==> review.tex <==
% !TEX root =  paper.tex

\subsection{Sequential Monte Carlo}
A good place to start is a brief review of sequential Monte Carlo as performed on state-space models. Given some latent random variables $X_{0}, …, X_{N}$ and some observed random variables $Y_{0}, …, Y_{N}$, we can describe the joint density: 

\[ p(x_{n} | x_{0:n-1}, y_{0:n-1}) = f(x_{n} | x_{0:n-1}) \]
\[ p(y_{n} | x_{0:n}, y_{0:n-1}) = g(y_{n} | x_{0:n}), \]

such that $X_{0}$ is sampled from an initial distribution $\mu(\cdot)$. $f$ and $g$ are conditional densities. 

Given observed values $Y_{0:N} = y_{0:N}$, a weighted set of $K$ particles is used to approximate the posterior distribution $p(x_{0:n} | y_{0:n})$ where each particle $k$ is written as $X_{0:n}^{k}$ for $k = 1, …, K$. At the next iteration, particles are propagated from proposal densities $q(x_{n} | x_{0:n-1})$ and reweighed at each $n = 1, …, N$: 

\[ X_{n}^{k} | X_{0:n-1}^{k} ~ q(x_{n} | X_{0:n-1}^{k}) \]
\[ w_{n}^{k} =  \frac{g(y_{n} | X_{0:n}^{k})f(X_{n}^{k} | X_{0:n-1}^{k})}{q(X_{n}^{k} | X_{0:n-1}^{k})} \]
\[ W_{n}^{k} = W_{n-1}^{k}w_{n}^{k}, \]

where $w_{n}^{k}$ is the observation $y_{n}$’s weight and $W_{n}^{k}$ is the unnormalized weight of particle $k$ after observation $n$. If simulating the system is possible, the proposal distribution can be chosen as $q(\cdot) \equiv f(\cdot)$, such that the particle weights are $w_{n}^{k} = g(y_{n} | X_{0:n}^{k})$. 

The normalized particle weights $\bar{w}_{n}^{k} = \frac{W_{n}^{k}}{\sum_{j=1}{K}W_{n}^{j}}$ are used to estimate the posterior:
\[ \hat{p}(x_{0:n} | y_{0:n}) \approx \sum_{k=1}^{K}\bar{w}_{n}^{k}\delta_{X_{0:n}^{k}}(x_{0:n}) \]

Given that this is simple sequential importance sampling, the marginal likelihood is estimated by $\hat{p}(y_{0:n}) = \frac{1}{K}\sum_{k=1}^{K} W_{n}^{k}$.

\subsubsection{Degeneracy and Resampling}
The sequential Monte Carlo algorithm generally suffers from a degeneracy problem wherein most of the normalized weights $\bar{w}_{n}^{-1}, ..., \bar{w}_{n}^{K}$ converge close to zero for even moderately large $n$. Because of this, a resampling step is added at each $n$. From step $n$ to $n+1$, particles with high weights are copied and particles with low weights are discarded in hopes of preventing all the probability mass in the posterior approximation to accumulate on a single particle. By resampling, the weights of the particles change: from step $n$ to $n+1$, each of the $M_{n+1}^{k}$ children are assigned a new weight $V_{n+1}^{k}$, instead of the previous weight $W_{n}^{k}$ prior to resampling. The resampling scheme used in this paper generates an unweighted set of particles with $V_{n+1}^{k} = 1$ for all particles. 
 
\subsubsection{Sample Impoverishment and Independent Inference Blocks}
The inference algorithm described above may converge to only a few values in the posterior approximation for a given latent variable, especially if the assumed prior distribution is poorly chosen. No model is perfect but especially poor parameters are highly susceptible to what is known as sample impoverishment, where all particles converge to as few as one value for a latent variable. This is undesirable since any user would expect the probabilistic system to produce a distribution. To prevent this, independent blocks of inference are introduced: instead of using sequential Monte Carlo on all $K$ particles, it is performed using $K_{r}$ particles for $r$ repetitions where 
\[K_{r} = \left\{\begin{matrix} K/r & \textup{if } k = 1, ..., r-1\\ K/r + K\%r & \textup{else if } k = r \end{matrix}\right.\]
With $r$ repetitions of sequential Monte Carlo, there are at least $r$ separate sets of $K_{r}$ particles, and $r$ different posterior approximations $\hat{p_{r}}(x_{0:n}|y_{0:n})$, reducing the probability of sample impoverishment. For each variable, the normalized particle weights $\bar{w}_{n}^{k}$ are used to approximate the posterior as a linear combination of particles with overlapping variable values in each block $r$.

\subsection{Black Box Variational Inference}
Variational inference looks at the problem of approximating a conditional distribution as an optimization problem [Jordan et al., 1999; Biship, 2006; Wainwright and Jordan, 2009]. Given a simple family of distributions over the latent variables of a state space, the goal is to find the member of the family that is closest in KL divergence to the conditional distribution. Let $x$ be observations, $z$ be latent variables, $\lambda$ be free parameters of the proposed $q(z|\lambda)$. To approximate $p(z|x)$, we can minimize the KL divergence by maximizing the ELBO, defined as:
\[ \mathcal{L}(\lambda) \doteq E_{q_{\lambda(z)}}[\textup{log} \ p(x, z) - \textup{log} \ q(z)] \]

Black Box Inference uses stochastic optimization to perform the optimization using noisy estimates of the gradient. Given some $f(x)$, the function to be maximized, and $h_{t}(x)$, a binding of a random variable $H(x)$ s.t. $E[H(x)] = $gradient$(f(x))$. If $\rho_{t}$ is a learning rate, then stochastic optimization is defined as:
\[ x_{t+1} \leftarrow x_{t} + \rho_{t}h_{t}(x_{t}) \]

This converges to a maximum when learning rate follows Robbins-Monro:
\begin{center}
	$\sum_{t=1}^{\infty} \rho_{t} = \infty$, $\sum_{t=1}^{\infty} \rho_{t}^{2} < \infty$
\end{center}

It is a black box method because the gradient of the of of the variational distribution and sampling method can be derived once for each type of variational distribution and reused for many different models. A noisy gradient of the ELBO is shown as an expectation with respect to the variational distribution: 
\[ \triangledown_{\lambda}\mathcal{L} = E_{q}[\triangledown_{\lambda} \textup{log} \ q(z|\lambda)(\textup{log} \ p(x, z) - \textup{log} \ q(z|\lambda))] \]

The algorithm repeats until the change in $\lambda < \varepsilon$. $\lambda_{1:n}$ is initialized randomly. To help convergence rates, control variates are implemented as described in \citet{ranganath2013black}. 

\subsection{AdaGrad}
To ensure that the learning rate is small when the variance of the gradient is large, we use AdaGrad to set $\rho$. AdaGrad defines $G_{t}$ as a matrix composed of the sum of the first $t$ iterations of outer products of the gradient vectors. 
\[ \rho_{t} = \eta\textup{diag}(G_{t})^{-1/2} \]
For each $\lambda_{i}$, there is an individual learning rate given that $|G_{t}| = |\lambda_{i}|$. Using AdaGrad, the Robbins-Monro constraint is satisfied. 

% ---------------------------------------------------------------------



\subsection{Spreadsheets As a Popular Programming Language}
Spreadsheets are one of the most widely used data processing systems by individuals and organizations alike. Estimates show that hundreds of millions of spreadsheets are created yearly \citep{panko2008spreadsheet} with 55 million active users in 2012 \citep{scaffidi2005estimating}. Surveys of 72 firms \citep{floyd1995managing} concluded that companies invest time into large, complex spreadsheets with an average of 6,000 cells and custom user-defined functionality \citep{john2003project}. They have proven to be high valued and crucial to decision-making in firms. \citet{gable1991spreadsheet} examined 402 non-trivial spreadsheets in a Singaporean construction company, and found that 59\% of the spreadsheets were referenced monthly. Additionally, \citet{chan1996use}, surveying 256 spreadsheet users, discovered that 42\% of them created spreadsheets used by the chief executive officer. Spreadsheets provide an easy way for organizations to make customized reports and extrapolate patterns from growing data sources. Due to their low barrier-to-entry and processing power, spreadsheets have steadily infiltrated into sports, finance, education, personal life, medicine, and more.

In addition to being popular, spreadsheets are a programming language, in fact, the most widely used one with 11 million end-user programmers  \citep{ko2011state}. These are small-businesses and independent experts in domains other than professional programming needing computational support for which spreadsheets are the primary way to obtain their goals. Possible scripts can range from simple mathematical calculations to complex financial models. Spreadsheets are therefore a program, with program defined as ``a collection of specifications that may take variable inputs, and that can be executed (or interpreted) by a device with computational capabilities.'' \citep{ko2011state}. By that definition, most programs written in world are not by professional software developers, but by these end-users.
And as with any program, a spreadsheet has inputs, outputs, and execution: In a classic spreadsheet system, a user can modify cells of values, references, and formulas. Cells that contain non-referenced constant values are equivalent to labels, providing documentation for the user. Cells that are referenced by others are comparable to inputs to the spreadsheet system, to be used by cells containing non-trivial formulas. These cells, possibly referencing other cells containing formulas, create a chain of computations. Finally, cells with formulas not referenced are the outputs. By changing certain cells, users are performing spreadsheet update operations, which can affect the execution or the inputs/outputs depending on the cell type. FOR and WHILE loops are replaced by column and row repetition where users can control the number of iterations. Additionally, looping can be performed with circular cell references: users can specify a maximum number of iterations or a value threshold. Because spreadsheets feature selection (functional if-then-else), composition (references), and repetition, they are indeed a simple programming language.

More formally, a spreadsheet is an applicative, first-order functional programming language. This means that the structure and elements of spreadsheets treat computation as the evaluation of mathematical functions and avoids using mutable data structures. In spreadsheets, the output value of a cell containing a function depends solely on the input arguments. Additionally, spreadsheets are purely composed of expressions, lack side effects, and its evaluation methods are declarative and controlled by data dependencies.



